Kinetic energy operator approach to the quantum three-body problem with Coulomb interactions

We present a non-variational, kinetic energy operator approach to the solution of quantum three-body problem with Coulomb interactions, based on the utilization of symmetries intrinsic to the kinetic energy operator, i.e., the three-body Laplacian operator with the respective masses. Through a four-step reduction process, the nine dimensional problem is reduced to a one dimensional coupled system of ordinary differential equations, amenable to accurate numerical solution as an infinite-dimensional algebraic eigenvalue problem. A key observation in this reduction process is that in the functional subspace of the kinetic energy operator where all the rotational degrees of freedom have been projected out, there is an intrinsic symmetry which can be made explicit through the introduction of Jacobi-spherical coordinates. A numerical scheme is presented whereby the Coulomb matrix elements are calculated to a high degree of accuracy with minimal effort, and the truncation of the linear equations is carried out through a systematic procedure

==> RPP/Tables/Helium/He1Pe.tex <==
\begin{table}
\scriptsize \caption{\label{table:He1Pe} Convergence study  for the
energies of the   five low-lying  ${}^{1}P^{e}$ states of ${}^\infty
\textrm{He}$ and $\textrm{He}$ }
\begin{tabular}{cccccc}
\hline
\hline
($M$, $N$, $P$)&$-E_0$&$-E_1$&$-E_2$&$-E_3$&$-E_4$\\
\hline\\
\multicolumn{6}{c}{${}^\infty \textrm{He}$}\\
(430,230,60)&.5802464721880898&.5400415791839888&.5241788416480129
&.5162076095833906&.5116198373348310\\
(450,240,60)&.5802464722667232&.5400415814536438&.5241788686149399
&.5162078008855000&.5116207852526047\\
(470,250,60)&.5802464723277703&.5400415832168637&.5241788895865377
&.5162079499058201&.5116215256596536\\
(490,260,60)&.5802464723756553&.5400415846007780&.5241789060623365
&.5162080671544037&.5116221095933119\\
(510,270,60)&.5802464724135769&.5400415856973018&.5241789191279953
&.5162081602594134&.5116225742579672\\
(530,280,60)&.5802464724438727&.5400415865737552&.5241789295794899
&.5162082348262304&.5116229470978563\\
(550,290,60)&.5802464724682687&.5400415872800159&.5241789380073016
&.5162082950213394&.5116232485822370\\
(570,300,60)&.5802464724880733&.5400415878533919&.5241789448544265
&.5162083439745614&.5116234941328116\\
(590,310,60)&.5802464725042583&.5400415883222315&.5241789504561283
&.5162083840606537&.5116236954795450\\
{Extrap.}\tnote{a}
&\multicolumn{1}{l}{.58024647259(4)}
&\multicolumn{1}{l}{.5400415909(3)}
&\multicolumn{1}{l}{.524178981(7)}
&\multicolumn{1}{l}{.51620860(9)}
&\multicolumn{1}{l}{.51162483(4)}\\
\multicolumn{6}{c}{$\textrm{He}$}\\
(430,230,60)&.5801657683190155&.5399671662640823&.5241068140045408&
.5161367556459259&.5115496499491888\\
(450,240,60)&.5801657683976442&.5399671685335237&.5241068409683716&
.5161369469254993&.5115505977498680\\
(470,250,60)&.5801657684586814&.5399671702965672&.5241068619376357&
.5161370959281751&.5115513380653313\\
(490,260,60)&.5801657685065617&.5399671716803559&.5241068784115652&
.5161372131630032&.5115519219255652\\
(510,270,60)&.5801657685444845&.5399671727767552&.5241068914757834&
.5161373062566177&.5115523865330368\\
(530,280,60)&.5801657685747768&.5399671736531116&.5241069019261063&
.5161373808144485&.5115527593282703\\
(550,290,60)&.5801657685991747&.5399671743592799&.5241069103529985&
.5161374410027255&.5115530607734217\\
(570,300,60)&.5801657686189716&.5399671749326176&.5241069171992706&
.5161374899501383&.5115533062924168\\
(590,310,60)&.5801657686351489&.5399671754013580&.5241069228004918&
.5161375300310985&.5115535076142314\\
{Extrap.}\tnote{a}
&\multicolumn{1}{l}{.58016576872(5)}
&\multicolumn{1}{l}{.5399671780(1)}
&\multicolumn{1}{l}{.524106954(1)}
&\multicolumn{1}{l}{.516137755(4)}
&\multicolumn{1}{l}{.511554646(4)}\\
\hline
\hline
\end{tabular}
\end{table}


==> RPP/Tables/Helium/He3Pe.tex <==
\begin{table}
\scriptsize \caption{\label{table:He3Pe}Convergence study for the
energies of the  five low-lying  ${}^{3}P^{e}$ states of ${}^\infty
\textrm{He}$ and $\textrm{He}$ }
\begin{tabular}{cccccc}
\hline
\hline
($M$, $N$, $P$)&$-E_0$&$-E_1$&$-E_2$&$-E_3$&$-E_4$\\
\hline\\
\multicolumn{6}{c}{${}^\infty \textrm{He}$}\\
(430,230,60)&.7105001556706697&.5678128978416493& .5358671688063325&
.5222543663940791&.5151588182839487\\
(450,240,60)&.7105001556721519&.5678128980124475&.5358671726558373&
.5222544066018652&.5151590818018635\\
(470,250,60)&.7105001556733056&.5678128981451042&.5358671756474780&
.5222544378852249&.5151592872036325\\
(490,260,60)&.7105001556742089&.5678128982491671&.5358671779963474&
.5222544624724999&.5151594489016945\\
(510,270,60)&.7105001556749242&.5678128983316138&.5358671798580391&
.5222544819780347&.5151595773664767\\
(530,280,60)&.7105001556754937&.5678128983974923&.5358671813464656&
.5222544975863092&.5151596802982401\\
(550,290,60)&.7105001556759534&.5678128984505620&.5358671825461548&
.5222545101764112&.5151597634245981\\
(570,300,60)&.7105001556763296&.5678128984936414&.5358671835204065&
.5222545204079131&.5151598310513219\\
(590,310,60)&.7105001556766264&.5678128985288620&.5358671843171375
&.5222545287806556&.5151598864509140\\
{Extrap.}\tnote{a}
&\multicolumn{1}{l}{.71050015567(8)}
&\multicolumn{1}{l}{.56781289872(5)}
&\multicolumn{1}{l}{.5358671887(7)}
&\multicolumn{1}{l}{.522254575(7)}
&\multicolumn{1}{l}{.515160198(3)}\\
\multicolumn{6}{c}{$\text{He}$}\\
(430,230,60)&.7103964575497739&.5677338692387791&.5357932647830638&
.5221825614509467&.5150880819401956\\
(450,240,60)&.7103964575512566&.5677338694095807&.5357932686322323&
.5221826016555502&.5150883454346265\\
(470,250,60)&.7103964575524059&.5677338695422228&.5357932716236884&
.5221826329364018&.5150885508180396\\
(490,260,60)&.7103964575533118&.5677338696462903&.5357932739723949&
.5221826575216685&.5150887125017813\\
(510,270,60)&.7103964575540251&.5677338697287290&.5357932758339309&
.5221826770257165&.5150888409551973\\
(530,280,60)&.7103964575545967&.5677338697946014&.5357932773223104&
.5221826926326127&.5150889438778797\\
(550,290,60)&.7103964575550581&.5677338698476703&.5357932785219116&
.5221827052217765&.5150890269968378\\
(570,300,60)&.7103964575554310&.5677338698907493&.5357932794960780&
.5221827154525562&.5150890946175062\\
(590,310,60)&.7103964575557372&.5677338699259572&.5357932802928009&
.5221827238245294&.5150891500082744\\
{Extrap.}\tnote{a}
&\multicolumn{1}{l}{.71039645755(7)}
&\multicolumn{1}{l}{.56773387012(2)}
&\multicolumn{1}{l}{.5357932847(4)}
&\multicolumn{1}{l}{.522182770(7)}
&\multicolumn{1}{l}{.51508946(19)}\\
\hline
\hline
\end{tabular}
\end{table}


==> RPP/figures.tex <==
\Figures
%%%**********************************************




%****************************************
%
%    Helium
%
%*****************************************

